Geometry-Aware Texture Generation for 3D Head Modeling with Artist-driven Control

Creating realistic 3D head assets for virtual characters that match a precise artistic vision remains labor-intensive. We present a novel framework that streamlines this process by providing artists with intuitive control over generated 3D heads. Our approach uses a geometry-aware texture synthesis pipeline that learns correlations between head geometry and skin texture maps across different demographics. The framework offers three levels of artistic control: manipulation of overall head geometry, adjustment of skin tone while preserving facial characteristics, and fine-grained editing of details such as wrinkles or facial hair. Our pipeline allows artists to make edits to a single texture map using familiar tools, with our system automatically propagating these changes coherently across the remaining texture maps needed for realistic rendering. Experiments demonstrate that our method produces diverse results with clean geometries. We showcase practical applications focusing on intuitive control for artists, including skin tone adjustments and simplified editing workflows for adding age-related details or removing unwanted features from scanned models. This integrated approach aims to streamline the artistic workflow in virtual character creation.

==> 1.intro.tex <==
\section{Introduction}
\label{sec:intro}

Populating virtual scenes with realistic-looking avatars with great diversity is crucial for creating an immersive user experience for a range of applications, including video games, cinematic productions, and virtual reality experiences. This entails creating head assets including geometry (the spatial coordinates of vertices) and intrinsic texture maps (diffuse, specular, and normal maps) necessary for realistic rendering.
However, generating diverse, realistic character heads at scale can be time-consuming for artists and often requires specialized skills in face modeling. This motivates research on convenient ways to generate and edit 3D head assets.

A common approach for head asset generation relies on 3D Morphable models (3DMM) \cite{blanz1999morphable}. 
These methods create a statistical model from a collection of head scans \cite{Egger20Years}. 
New heads can be generated by linearly combining bases from the statistical model. While convenient, 3DMMs tend to produce overly smooth results that lack detail.
This motivated research on Non-linear Morphable Models using Generative Adversarial Networks \cite{goodfellow2014generative} to produce more detailed heads \cite{li2020learning, rai2023towards}, including intrinsic texture maps (such as diffuse, specular and normal maps). 
However, these models are generally difficult to train and are prone to produce artifacts during generation. To leverage Convolutional Neural Networks (CNN), they represent geometry in a canonical space by projecting the 3D vertex positions onto a 2D UV map, which has significant drawbacks. Mainly, it is not possible to unwrap a 3D Head geometry to 2D without any cuts. This causes some vertices that are close in the 3D space to appear far in the 2D UV space. Additionally, depending on the UV parametrization, vertices of facial features such as the mouth and eye contours, may be close in UV space, but far in 3D space, which results in artifacts during generation.
For this reason, methods that estimate geometry in UV-space rely on post-processing steps. For instance, in \cite{li2020learning}, a separate linear model is applied to problematic areas (mouth and eye contours), which are later integrated into the geometry produced by the non-linear generator.
Conversely, non-linear methods relying on Graph Neural Networks (GNNs) \cite{COMA:ECCV18},  operate directly on the vertex-level, and thus do not share this limitation. These methods are capable of generating complete heads without post-processing steps. Since they operate on vertex level, however, they are not suitable for generating detailed texture maps, often represented as high-resolution images (e.g. 4k or 8k in modern games and films).

Recent approaches, linear as well as non-linear, do not allow users to interact with the model for precise manipulation of the produced head. For instance, some methods \cite{lattas2023fitme, lattas2021avatarme++, papantoniou2023relightify} are conditioned on images, which requires manipulating face attributes in the input image space in the hope that the model will accurately reproduce the details in the 3D head. Similarly, systems conditioned on text prompts \cite{zhang2023dreamface, wang2023rodin} allow users to change face attributes on a global level, but do not allow to specify the exact location of a scar or a mole. Moreover, sometimes words can fail to precisely describe a skin tone or facial features such as the shape of the eyebrows. This limits the usability of these techniques in high-end tools for projects with specific artistic intents and constraints.

In this work, we introduce a novel framework for generating 3D heads tailored to provide artists with precise control over the generated assets. Our approach combines a GNN-based model for generating geometry at the vertex level coupled with a texture generator that uses a CNN to generate intrinsic 2D texture maps.
Notably, we propose a geometry-aware texture generation process that, by design, is capable of learning correlations between head geometry and skin texture (e.g. due to ethnicity, gender, and age). To enable artistic control, we design a texture generation pipeline that enables:
(i) precise control of skin tone generation, and (ii) adding/removing fine-grained details such as wrinkles. 
%Skin-tone control is achieved with a novel data-driven approach, using an intermediate representation for skin textures. 
%that learns a transformation from melanin maps and skin color maps. 
This is achieved through a novel method that separates high- and low-frequency skin attributes, enabling independent control over skin tone and fine-grained details. Moreover, these modifications are cohesively propagated to the intrinsic texture maps (diffuse, specular, and normal), significantly reducing artists’ workload, as they only need to edit a single map.

We make the following contributions:
%\ad{contrib: reduire le bias ... a voir}
\begin{itemize}
    
    %\item We introduce a new head generation model that includes a geometry-aware texture generator, that is capable of learning correlations between head geometry and texture.
    
    \item We propose a framework for complete 3D head generation that allows for user control at three different levels.
    
    \item We combine a GNN-based Variational Autoencoder (VAE) for geometry generation with a geometry-aware texture generator. This enables the creation of high-quality head assets with clean meshes, eliminating the need for post-processing.
    %\ad{with separate control path for skin tone and fine grained details?}
    %without artifacts in the geometry, without post-processing.}

    \item We introduce a novel approach for editing fine-grained details in intrinsic texture maps. This allows artists to modify a single texture map using any image editing tool, with the changes coherently propagated to the intrinsic texture maps. 

    \item We present a data-driven method that allows precise manipulation of skin tones while preserving other aspects of the texture. %\ad{This allows also to compensate for bias?? the first method?}
\end{itemize}
%
\begin{comment}
Context:
\begin{itemize}
    \item Realistic virtual human representation is central for a range of applications: Video games, VFX, animation, meta verse
    \item Modeling realistic human looking is time consuming (light stage) and requires skilled artists and engineers. (also manual sculpting z brush) (faster convergence?)
    % \item To achieve realistic rendering, modern engines uses multiple rendering layers: 
    % \begin{itemize}
    %     \item Full reflectance model (micro facet)
    %     \item Details map (displacement map or normal map)
    %     \item Sub surface scattering map
    %     \item Ambiant occlusion 
    % \end{itemize}
    \item Linear morphable models fall short in terms of quality and does not meet production requirements (low frequency aspect of PCA, low resolution reflectance model bound by the statistical albedo model).
    \item Can we say something about controlability.
    Rodin (implicit representation). DreamFAce (outputs a mesh from a prompt)
    \item Other methods like ICT does not provide artist control on the output. (no artist control on the generated map)  We can also cite here GanFit and it is limitation (lack realism and restricted generative model) 
    \item Most of these existing non linear models are trained on smaller datasets. While our method can be trained on more data 
\end{itemize}


Contributions: 

\begin{itemize}
    %\item  (Laplacian 2D/3D) we propose an improved training scheme that produces detailed meshes compared to sota by leveraging the mesh laplacain during training  (use laplacian 2D as a new fid evaluation metric)

    \item We propose improved strategies for training non-linear face geometry generators. The new formulations make training more stable and converge faster, generating meshes with fewer artifacts and more diversity.
    
    %\item new metric more  face genetatros based on laplacain and diff rendering    

    \item We derive a new albedo representation based on a novel artist-driven melanin/hemoglobin representation which provides control on the generated albedo (darker/white skin) (revised?) and edges
    % section that shows how to combine these maps into albedo; how to decompose an existing albedo into two components that allow this manipulation  
    % Show that changing melanin power -> change skin tone without changing anything else

    \item We propose a new way of manipulating fine-grained details on skin textures, allowing the manipulation of a single edge map that propagates changes in all texture maps used to render realistic faces.
    
\end{itemize}

\begin{itemize}
\item The first 3D face non linear generative model that produces production ready assets including: Diffuse, specular and roughness maps Displacement map AO, SSS at 4K
\item We derive a new albedo representation based on a novel artist-driven melanin/hemoglobin representation which provides control on the generated albedo (darker/white skin) (revised?)
%\item A novel data augmentation scheme that allows to train our model on large dataset. For instance, the aforementioned melanin representation allows us to generate large scale dataset (by mixing and blending different textures) and perform efficient data augmentation
%\item differentiable rendering ? (derive a new differentiable shading suitable for the inverse rendering problems) (for the evaluation)
\item (Laplacian 2D/3D) we propose an improved training scheme that produces detailed meshes compared to sota by leveraging the mesh laplacain during training  (use laplacian 2D as a new fid evaluation metric)  \item new metric more  face genetatros based on laplacain and diff rendering
\item sell the idea of controlable genetative models for artists. 
\item [TODO] put the geneator inside a face reconstructor network architecture and train a 3D face reconstrution from images
\end{itemize}
\end{comment}

%Non-linear Morphable Models that uses StyleGAN architecture \cite{Karras2019stylegan2} produce more detailed heads \cite{li2020learning, rai2023towards} and intrinsic texture maps (such as diffuse, specular and normal maps). 
%However, training such models is challenging and often leads to artifacts in the generation. These methods represents geometry in a canonical space, achieved by projecting the 3D vertex position onto a 2D UV-map, enabling the use of Convolutional Neural Networks (CNN). However, this approach presents significant drawbacks. 

%Moreover, both  approaches have limited control over the generation process and not provide any sort of fine grained control over the generated heads.}

%\ad{especially normal map required for detailed and realistic rendering.}

%These methods represent the geometry in a  canonical space by projecting the 3D vertex position to a 2D UV-map which allows the use of  Convolutional Neural Networks (CNN). However, this has some major drawbacks. For instance, cavities such as eye sockets and mouth are close in UV space but far in 3D space, which causes artifacts in the generation. To address this problem,  a post-processing step is applied on the generated mesh, by using an separate linear model for these areas, which is then stitched to the non-linear geometry of the generator to avoid seams. On the other hand, non-linear methods that use Graph Neural Networks (GNN) \cite{COMA:ECCV18} do not suffer from this limitation and can produce a complete head. However, because GNN operates on vertex level, they cannot  produces over smoothed texture skin reflectance maps.  color maps res  
%More recently, text prompts are used to condition generation \cite{zhang2023dreamface, wang2023rodin}. While this provides unconstrained high-level control over head characteristics, they requires prompting skills to achieve the desired output.  This limitation restricts its applicability for artists who frequently require precise control over the details of the generated heads.


%An alternative approach involves using linear generative models, specifically 3D Morphable Models (3DMM) \cite{blanz2023morphable}, for avatar generation. With 3DMM, new faces are generated through  a linear combination of the Principal Component Analysis (PCA) basis. However the quality of the output tends to be smooth smooth and may not meet the standards required for production. Moreover, these models do not offer any explicit control for artists to control or fine-tune the generation. 
%TODO: cite albedoGAN


%\cite{li2020learning, rai2023towards} that rely on Stylegan \cite{Karras2019stylegan2} and more recently, diffusion models  that can guided by text prompts. While some of  these methods produces realistic looking heads, they may fall short in providing enough control for editing and interaction that is compatible with the artist's workflow. For instance, guiding diffusion models through text prompts is still challenging and does not always yield the desired output. 



